An Industry Evaluation of Embedding-based Entity Alignment

Embedding-based entity alignment has been widely investigated in recent years, but most proposed methods still rely on an ideal supervised learning setting with a large number of unbiased seed mappings for training and validation, which significantly limits their usage. In this study, we evaluate those state-of-the-art methods in an industrial context, where the impact of seed mappings with different sizes and different biases is explored. Besides the popular benchmarks from DBpedia and Wikidata, we contribute and evaluate a new industrial benchmark that is extracted from two heterogeneous knowledge graphs (KGs) under deployment for medical applications. The experimental results enable the analysis of the advantages and disadvantages of these alignment methods and the further discussion of suitable strategies for their industrial deployment.

==> TODO <==
\revise{preprocess}

\add{D-W-15K-V2： 对于实体名字，由于实体是url形式，因此实体的名字取URL的最后一个部分，同时将“_”替换成空格；对于实体属性，将属性值按'^^'和'@en'截断，取前一部分。然后把'.(),"'全部去掉，把'_-/'替换成空格。这是rdf的格式，是为了取得属性值的有意义部分。这是OpenEA的做法。工业数据集：由于工业数据集不是url的形式，因此实体名字和属性直接和上面一样处理标点符号就行。所有的字母都会转成小写。}

\revise{industry data generation}

\add{数据来源：腾讯健康有一些问诊，miyin，搜一搜，医生信息（用户输入，医生回答，对话数据）；医院给的信息，包括主诉，病例，诊断；还有一些药品信息，花钱买的，比如美康；还有一些爬虫数据，比如9939，医生问答，爬虫（快速问医生），来源可能有10多个；}

数据来源-预处理{分类器，区分医学和非医学句子；爬虫：1，2，乱码啥的都过滤；格式预处理}-算法提取{ner，nre}，统计节点关系的频率，然后知识校验{词频过滤，来源判断正确与否：可以检测冲突}-link predict增加关系 属性的提取：结构化的属性，关系拿了一些做属性，爬的时候就自带属性

找到合适来源-数据预处理{结构化切割，分号，非医学脏数据取出}-算法找关系和属性-图谱补全{relation predict}-知识校验{词频，冲突}

mapping
从工业数据集的来源找到24k，然后用名字匹配在百度百科里找对齐的实体


==> sections/04-setting.tex <==

Besides the industrial benchmark, we also develop a new approach to extract biased seed mappings that match the industrial context.
% To extract the named biased seed mappings, we first calculate the name similarity score of the entities of each mapping, denoted as $s_{name}$ which is in $\left[0,1\right]$.
% Specifically $s_{name}$ is the normalized Levenshtein Distance -- an edit distance metric \cite{navarro2001guided} of the two name strings.
% The seed mappings with an attribute bias is calculated in a similar way.
% We calculate the average number of attributes of the entities of each mapping, denoted as $n_{attr}$, and rank all the mappings from more attributes to less attributes.

We firstly introduce two variables, $s_{name}$ and $n_{attr}$, in which $s_{name}$ is the normalized Levenshtein Distance -- an edit distance metric \cite{navarro2001guided} of the two name strings and $n_{attr}$ is the average number of attributes of each mapping.

Based on $s_{name}$ and $n_{attr}$, we divide benchmarks into three different splits from name-biased aspect and attribute-biased aspect.
From name-biased aspect, the benchmarks are divided into ``same'' ($s_{name} == 1.0$), ``close'' ($s_{name} < 1.0$) and ``different'' ($s_{name}$ is NA as any entity name is garbled).
From attribute-based aspect, the three splits include ``large'' ($n_{att} \geq k_1$), ``medium'' ($k_2 \leq n_{att} < k_1$) and ``small'' ($n_{att} < k_2$), where $(k_1,k_2)$ are set to $(5,2)$ for MED-BBK-9K and set to $(10,4)$ for D-W-15K.

With aforementioned splits, we detail our sampling strategy for biased seed mappings. 

% We then rank all the mappings from high similarity to low similarity, and select the top $\alpha\%$ (e.g., $6\%$) as seed mappings for training and validating, and the remaining for testing.

% Meanwhile, to further analyze the impact of the seed mapping on different testing mappings, we divide the testing mappings into $3$ splits according to the name similarity score ($s_{name}$) or the average attribute number ($n_{attr}$), and measure Hits@$1$ within each testing split.
% When the name similarity score is used for splitting, the three sets are ``same'' ($s_{name} \geq 1.0$), ``close'' ($0.9 \leq s_{name} < 1.0$) and ``different'' ($s_{name} < 0.9$) for both MED-BBK-9K and D-W-15K. 
% When the average attribute number is used for splitting, the three sets are ``large'' ($n_{att} \geq k_1$), ``medium'' ($k_2 \leq n_{att} < k_1$) and ``small'' ($n_{att} < k_2$), where $(k_1,k_2)$ are set to $(5,2)$ for MED-BBK-9K and set to $(10,4)$ for D-W-15K.

\add{
1. We design a scoring function for each mapping that $z(e_1, e_2) = z_{name} + z_{attr}$ where $z_{name} = z_{attr} = 4$ if the mapping is in ``same'' split or ``large'' split, $z_{name} = z_{attr} = 3$ if the mapping is in ``close'' split or ``medium'' split, and $z_{name} = 1$ if the mapping is in ``different'' split or ``small'' split. All the mappings are divided into different sets with score of 8, 7, 6, 5, 4, or 2. 

2. Starting from high-score sets, the corresponding entity pairs are appended into an empty set, called biased set.

3. Check if the number of mappings in the biased set is enough to sample training/validation data (e.g., $6\%$ of all the mappings). If yes, we randomly sample a certain proportion of the biased set to obtain training/validation sets, and set the rest of mappings as test set for evaluation. If no, return to Step 2, continue to append following low-score sets into the biased set, and proceed the iteration.
}

We obtain solely name-biased seed mappings with the scoring function $z(e_1, e_2) = z_{name}$ and attribute-based seed mappings with the scoring function $z(e_1, e_2) = z_{attr}$ in the above strategy
